$\mathcal{N}$IPM-MPC: An Efficient Null-Space Method Based Interior-Point Method for Model Predictive Control

Linear Model Predictive Control (MPC) is a widely used method to control systems with linear dynamics. Efficient interior-point methods have been proposed which leverage the block diagonal structure of the quadratic program (QP) resulting from the receding horizon control formulation. However, they require two matrix factorizations per interior-point method iteration, one each for the computation of the dual and the primal. Recently though an interior point method based on the null-space method has been proposed which requires only a single decomposition per iteration. While the then used null-space basis leads to dense null-space projections, in this work we propose a sparse null-space basis which preserves the block diagonal structure of the MPC matrices. Since it is based on the inverse of the transfer matrix we introduce the notion of so-called virtual controls which enables just that invertibility. A combination of the reduced number of factorizations and omission of the evaluation of the dual lets our solver outperform others in terms of computational speed by an increasing margin dependent on the number of state and control variables.

==> 202104_mpcIntPtPaper (copy)/commands.tex <==

% Math specific
\newcommand{\vect}[1]{\mathbf{#1}}                  %vector
\newcommand{\greekvect}[1]{\bm{#1}}                 %greek letter vector
\newcommand{\const}[1]{\mb{#1}}                     %constante
\newcommand{\inv}{^{\text{-}1}}                     %inverse
\newcommand{\tp}{\ensuremath{^{\mathsf{T}}}}		%transpose
\newcommand{\superM}{^{\text{-}}}                   %Superscript minus
\newcommand{\superP}{^{\text{+}}}                   %Superscript plus
\newcommand{\minus}{\text{-}}                       %Minus in front
\renewcommand{\exp}[1]{\mathrm{e}^{#1}}             %Exponential
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\card}{card}

\newcommand{\nextinc}{^{(k+1)}}
\DeclareMathOperator*{\mini}{min.}
\DeclareMathOperator*{\lexmin}{lexmin.}
%\newcommand\myeq{\hspace{3pt}\stackrel{\mathclap{\normalfont\mbox{def}}}{=}\hspace{3pt}}
\newcommand\myeq{\hspace{3pt}\stackrel{\text{def}}{=}\hspace{3pt}}
\definecolor{light-gray}{gray}{0.95}
\definecolor{dark-gray}{gray}{0.5}
\definecolor{mygray}{gray}{0.75}
\newcommand{\BIN}{\begin{bmatrix}}
\newcommand{\BOUT}{\end{bmatrix}}
\newcommand{\cur}{^{(k)}}
\newcommand{\pre}{^{(k-1)}}
\newcommand{\nextopt}{^{(k+1)*}}
\newcommand{\ue}{\underline{e}}
\newcommand{\uw}{\underline{w}}
\newcommand{\uv}{\underline{v}}
\newcommand{\uW}{\underline{W}}
\newcommand{\uV}{\underline{V}}
\newcommand{\uJ}{\underline{J}}
\newcommand{\uH}{\underline{H}}
\newcommand{\ulambda}{\underline{\lambda}}
\newcommand{\uLambda}{\underline{\Lambda}}
\newcommand{\uA}{\underline{A}}
\newcommand{\tA}{\tilde{A}}
\newcommand{\utA}{\underline{\tilde{A}}}
\newcommand{\umA}{\underline{\mathcal{A}}}
\newcommand{\ub}{\underline{b}}

% Writing command
\newtheorem{Def}{Definition}
\def\al{~\textit{et al. }}
\def\eg{\textit{e.g.}~}
\def\ie{\textit{i.e.} }
\def\resp{\textit{resp.} }

% Reference command
\newcommand{\Annref}[1]{Appendix~\ref{#1}}
\newcommand{\Eqref}[1]{Eq.~\eqref{#1}}
\newcommand{\Eqrefand}[2]{Eq.~\eqref{#1} and~\eqref{#2}}
\newcommand{\Eqrefrange}[2]{Eq.~\eqref{#1}~\text{--}~\eqref{#2}}
\newcommand{\Figref}[1]{Fig.~\ref{#1}}
\newcommand{\Figrefand}[2]{Fig.~\ref{#1} and~\ref{#2}}
\newcommand{\Figrefrange}[2]{Fig.~\ref{#1}~\text{--}~\ref{#2}}
\newcommand{\SubFigref}[1]{(\subref{#1})}
\newcommand{\SubFigrefrange}[2]{(\subref{#1})~\text{--}~(\subref{#2})}
\newcommand{\Chpref}[1]{Chapter~\ref{#1}}
\newcommand{\Secref}[1]{Section~\ref{#1}}
\newcommand{\Secrefand}[2]{Section~\ref{#1} and~\ref{#2}}
\newcommand{\Secrefrange}[2]{Section~\ref{#1}~\text{--}~\ref{#2}}
\newcommand{\Problemref}[1]{Problem~(\ref{#1})}
\newcommand{\Algoref}[1]{Algorithm~(\ref{#1})}
\newcommand{\Appref}[1]{Appendix~\ref{#1}}
\newcommand{\Tableref}[1]{Table~(\ref{#1})}

%\floatname{algorithm}{Algorithm}
%\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicensure}{\textbf{Output:}}

\pgfdeclarelayer{bg1}   
\pgfdeclarelayer{bg}  
\pgfsetlayers{bg1,bg,main}  

\setcounter{secnumdepth}{3}  
\setcounter{tocdepth}{3}     

\definecolor{orange}{rgb}{0.99,0.69,0.07}
\definecolor{lightgray}{gray}{0.85}
\definecolor{light-gray}{gray}{0.95}
\definecolor{dark-gray}{gray}{0.5}


\tikzset{cross/.style={cross out, draw=black, minimum size=2*(#1-\pgflinewidth), inner sep=0pt, outer sep=0pt},
%default radius will be 1pt. 
cross/.default={1pt}}

%\newtheorem{definition}{Definition}[section]

% Modification notice
\newcommand{\aRemplir}[1]{------------------------------------ A remplir : #1-----------------------------------------}
%\newenvironment{todo}{\color{blue}\%}{\%}
\newcommand{\afaire}[1]{{\color{blue}\%TODO. #1}}

 \makeatletter
 \newcommand\fs@spaceruled{\def\@fs@cfont{\bfseries}\let\@fs@capt\floatc@ruled
   \def\@fs@pre{\vspace{5pt}\hrule height.8pt depth0pt \kern2pt}%
   \def\@fs@post{\kern2pt\hrule\relax}%
   \def\@fs@mid{\kern2pt\hrule\kern2pt}%
   \let\@fs@iftopcapt\iftrue}
 \makeatother
 
 \newcommand\blfootnote[1]{%
   \begingroup
   \renewcommand\thefootnote{}\footnote{#1}%
   \addtocounter{footnote}{-1}%
   \endgroup
 }
 
 \newcommand{\tabitem}{%
   \usebeamertemplate{itemize item}\hspace*{\labelsep}}
